PipeDream: Fast and Efficient Pipeline Parallel DNN Training

PipeDream is a Deep Neural Network(DNN) training system for GPUs that parallelizes computation by pipelining execution across multiple machines. Its pipeline parallel computing model avoids the slowdowns faced by data-parallel training when large models and/or limited network bandwidth induce high communication-to-computation ratios. PipeDream reduces communication by up to 95% for large DNNs relative to data-parallel training, and allows perfect overlap of communication and computation. PipeDream keeps all available GPUs productive by systematically partitioning DNN layers among them to balance work and minimize communication, versions model parameters for backward pass correctness, and schedules the forward and backward passes of different inputs in round-robin fashion to optimize "time to target accuracy". Experiments with five different DNNs on two different clusters show that PipeDream is up to 5x faster in time-to-accuracy compared to data-parallel training.

==> tex/api-table.tex <==
\begin{comment}
%[tufte!]
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{p{4cm}|p{4cm}}

Function  & Description\\
\hline
GetWork() & mini-batch id to process (forward or backward)\\
ReadParameters(LayerID, staleness) & Returns buffer filled with model parameters\\
PrepareUpdate(LayerID) & Returns buffer for recording the gradient\\
GetActivations(LayerID, MinibatchID) & Returns buffer with layer activations\\
PrepareOutput(LayerID, MinibatchID) & Returns buffer for recording layer output\\
LayerCompleted(LayerID, MinibatchID) & Releases layer input and output buffers

\end{tabular}
\caption{{\small \system{} API}}
\label{table:fiddle-api-1}
\end{table}
\end{comment}


\begin{comment}

\begin {table*}[t]\small
\begin{center}
  \begin{tabular}{| l | l |}
    \hline
    {\small \textbf{Function Name}}& 
    {\small \textbf{Description} } 
    \\ \hline
    \texttt{GetWork()} & 
    {\small Mini-batch ID to process (forward or backward)} 
    \\ \hline
    \texttt{ReadParameters(LayerID, staleness)} & 
    {\small Returns buffer filled with model parameters} 
    \\ \hline
    \texttt{PrepareUpdate(LayerID)} & 
    {\small Returns buffer for recording the gradient } 
    \\ \hline
    \texttt{GetActivations(LayerID, MinibatchID)} & 
    {\small Returns buffer with layer activations } 
    \\ \hline
    \texttt{PrepareOutput(LayerID, MinibatchID)} & 
    {\small Returns buffer for recording layer output } 
    \\ \hline
    \texttt{LayerCompleted(LayerID, MinibatchID)} & 
    {\small Releases layer input and output buffers } 
    \\ \hline
  \end{tabular}
  \vspace{-0.075in}
  \caption{
    \small
    \label{table:fiddle-api}
    The \system{} runtime's API for interaction with the ML worker thread}
\end{center}
\vspace{-0.2in}
\end {table*}

\end{comment}



\begin {table}[t]\small
  \begin{tabular}{l}
    \hline
    {\small \textbf{\texttt{Function Name}}} and {\small \textbf{Description} } 
    \\ \hline
    \texttt{GetWork()} 
    \\  \hspace{0.1in} \--- {\small Mini-batch ID to process (forward or backward)} 
    \\ %\hline
    \texttt{ReadParameters(LayerID, staleness)}
    \\  \hspace{0.1in} \--- {\small Returns buffer filled with model parameters} 
    \\ %\hline
    \texttt{PrepareUpdate(LayerID)}
    \\  \hspace{0.1in} \--- {\small Returns buffer for recording the gradient } 
    \\ %\hline
    \texttt{GetActivations(LayerID, MinibatchID)}
    \\  \hspace{0.1in} \--- {\small Returns buffer with layer activations } 
    \\ %\hline
    \texttt{PrepareOutput(LayerID, MinibatchID)}
    \\  \hspace{0.1in} \--- {\small Returns buffer for recording layer output } 
    \\ %\hline
    \texttt{LayerCompleted(LayerID, MinibatchID)}
    \\  \hspace{0.1in} \--- {\small Releases layer input and output buffers } 
    \\ \hline
  \end{tabular}
  \vspace{-0.075in}
  \caption{
    \small
    \label{table:fiddle-api}
    APIs for interaction with ML worker thread}
\vspace{-0.2in}
\end {table}

==> tex/cdf-graphs.tex <==

\begin{figure}[t!]
  \centering 
  \begin{subfigure}{0.49\columnwidth} {
    \centerline{\includegraphics[width=1.0\columnwidth]{graphs/Inception-BN_Feature_Map_Size_cdf.pdf}}
    \caption{CDF of Feature Map size}
    \label{fig:inception-imagenet-feature-cdf}
  }
  \end{subfigure}
  \begin{subfigure}{0.49\columnwidth} {
     \centerline{\includegraphics[width=1.0\columnwidth]{graphs/Inception-BN_Layer_Times_cdf.pdf}}
    \caption{CDF of Layer times}
    \label{fig:inception-imagenet-times-cdf}
   }
  \end{subfigure}
  \caption{Inception-BN with ImageNet}
\end{figure}

\begin{figure}[t!]
  \centering
  \begin{subfigure}{0.49\columnwidth} {
    \centerline{\includegraphics[width=1.0\columnwidth]{graphs/VGG_Feature_Map_Size_cdf.pdf}}
    \caption{CDF of Feature Map size}
    \label{fig:vgg-imagenet-feature-cdf}
  }
  \end{subfigure}
  \begin{subfigure}{0.49\columnwidth} {
    \centerline{\includegraphics[width=1.0\columnwidth]{graphs/VGG_Layer_Times_cdf.pdf}}
    \caption{CDF of Layer times}
    \label{fig:vgg-imagenet-times-cdf}
  }
  \end{subfigure}
  \caption{VGG with ImageNet and CIFAR10}
\end{figure}


==> tex/communication-to-compute-graph.tex <==
\begin{figure}[t!]
  \centerline{\includegraphics[width=0.9\columnwidth]{graphs/comv_v_comm_no_cifar.pdf}}
  \vspace{-0.1in}
  \caption{
  \small
  Breakdown of time for different DNNs training on the \imagenet{} dataset.  The labels atop each bar indicates the configuration---A and B indicate which 4-machine cluster was used and the number indicates the number of images per minibatch. \clusterA{} is a fast and dedicated private cluster.
  \clusterB{} consists of public cloud GPU instances.
  }
  \label{fig:comp-commn}
  %\vspace{-0.2in}
\end{figure}

==> tex/discussion.tex <==
\section{Discussion}
\aaron{seems like we should drop all of this}

\label{sec:discussion}
\textbf{Models with Large Solution State.}
\aaron{I used pretty much all of this information in Sec~\ref{sec:motivation-data-parallel-sucks}}
As shown in Sec.~\ref{sec:eval}, data-parallel
scales poorly for models that have large parameter 
data size. For such models, pipeline-parallel 
can provide large improvements in training 
such as the ones observed for VGG16. Due to 
resource constraints we were unable to so far experiment
with other popular convolutional models including
Resnet-152 and Resnet-269~\cite{he2016deep}
which have parameter data size of $\sim$250MB and $\sim$390MB 
respectively.
Inception-V4~\cite{szegedy2017inception} has a parameter
data size $\sim$150MB. LSTM RNN models, which are commonly used 
for many tasks including language translation and video
classification tend to have even larger parameter data sizes,
making them difficult to train in data-parallel configurations.
Seq-2-Seq, a popular LSTM model, has a parameter data size
of $\sim$1.52GB. We plan on exploring these models in future work.

\textbf{Combining Data-Parallel and Pipeline-Parallel.}
\aaron{new section 4.5 kind of covers this, we don't have much interesting to 
say about this anyway}
\system{}'s current work splitting algorithm (Sec.~\ref{sec:design-work-distribution}) currently 
distributes work only in a straight-pipeline configurations.
Some neural network models, have large intermediate data 
in the bottom layers of the network, while having little
parameter data in those layers~\cite{krizhevsky2014one}.
For these models, combining data-parallelism with pipeline-parallelism could provide the best performance.
Data-parallelism would be used at the bottom of the network, since there is less parameter data to communicate in those layers, and then transition pipeline-parallelism as the 
the amount of parameter data increases. In future work,
we plan to modify \system{}'s work distribution algorithm,
to optimize for recommending configurations consisting of both
data-parallelism and pipeline-parallelism.

\textbf{Scaling Pipeline Parallel.}
\aaron{not much here}
Due to resource constraints, we have yet to be able to experiment
with scaling \system{} to more than four machines in pipeline-parallel
configurations. Most neural networks have large amount of layers (e.g Inception-BN has 248 layers) indicating it's possible to scale pipeline-parallel.


==> tex/eg_fig.tex <==
\section{Figures}
\label{sec:figs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
  \centerline{\includegraphics[width=0.95\columnwidth]{figs/stack.pdf}}
  \caption{Protocol stack of distributed transaction commit service}
  \label{fig:softwarestack}
\end{figure}



==> tex/eg_table.tex <==
\section{Tables}
\label{sec:tab}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular_environment

\newcolumntype{C}{>{\centering\arraybackslash}p{12mm}}
%\newcolumntype{C}{>{\centering}p{12mm}@{}}  % use \tabularnewline instead of \\ in tables

\begin{center}
\begin{tabular}{|C|c|C|C|}
\hline%
1A &\multirow{2}{12mm}{\centering W} & 1 & 2 \\
\cline{1-1} \cline{3-4}%
1B&                                  & 3 & 4 \\
\hline%
2A &\multirow{2}{12mm}{\centering Y} & 5 & 6 \\
\cline{1-1} \cline{3-4}%
2B &                                 & 7 & 8 \\
\hline%
\end{tabular}
\end{center}




\begin{comment}
%\usepackage{multicol}  % causes problem with paper title when in two-column mode

\begin{center}
%\begin{tabular}{|m{0.1\columnwidth}|m{0.2\columnwidth}|m{0.1\columnwidth}|m{0.35\columnwidth}|} 
\begin{tabular}{|l|l|l|l|} 
\hline
Index & \multicolumn{3}{|c|}{Schedulers} \\
\hline
\multirow{3}{*}{1} & \multirow{3}{*}{Immediate}    & RR & Round Robin \\
\cline{3-4}%
                   &                               & EF & Earliest First \\
\cline{3-4}%
                   &                               & LL & Lightest Loaded \\
\hline
\multirow{5}{*}{2} & \multirow{5}{*}{Batch}        & MM & Min-Min \\ 
\cline{3-4}%
                   &                               & MX & Max-Min \\
\cline{3-4}%
                   &                               & DL & Dynamic Level \\ 
\cline{3-4}%
                   &                               & RC & Relative Cost \\
\cline{3-4}%
                   &                               & \multicolumn{2}{c|}{YAY} \\
\hline
\multirow{4}{*}{3} & \multirow{4}{*}{Evolutionary} & PN & This paper \\
                   &                               & ZO & Genetic Algorithm\\
                   &                               & TA & Tabu search\\
                   &                               & SA & Simlulated Annealing \\
\hline
\end{tabular}
\end{center}

\end{comment}



\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{0.12\textwidth}|p{0.28\textwidth}|p{0.5\textwidth}}
Protocol & Safety Spec & Liveness Spec (for $\leq N$ failures)\\
\hline
Two Phase Commit & \textit{Atomicity} & Coordinator makes progress\\\hline
Chain Repl. & All invariants in~\cite{Renesse:osdi2004}, cmd-log consistency &  With stable head node, every cmd is eventually responded to\\\hline
Multi-Paxos & Consensus requirements \cite{Lamport:paxos-simple}, log consistency~\cite{VanRenesse:2015} & For a live quorum of replicas with all nodes trusting the leader has not failed, if the network is eventually synchronous, every proposal is eventually chosen.
%With stable leader, every proposal is always eventually learnt by learners\\\hline
%Basic Paxos & All consensus requirements in \cite{Lamport:paxos-simple} & With distinguished proposer, a proposal is eventually chosen \\
\end{tabular}
\caption{Example specifications checked for each protocol. SMR protocols are configured to be $N$ fault-tolerant}
\label{tab:specifications}
\end{table*}



\begin{table}[tbh]
\centering
\scriptsize
\begin{tabular}{l|c|c|c}
%\hline
Protocols \ & Unhandled & \multicolumn{2}{c}{Spec. Violation}\\
\hhline{~~--}
Components & Event & Safety & Liveness\\\hline
Two Phase Commit & 20 & 15 & 4\\
Chain Repl. & 26 & 10 & 7\\
Multi-Paxos & 10 & 22 & 3\\
Basic Paxos & 6 & 6 & -\\
Leader Election & 9 & - & -\\
View Membership & 10 & 8 & 1\\
Fault Detector & 6 & 4 & - \\
\hline
%\hhline{=====}
\textbf{Total (167)}& 87 & 65 & 15\\
%\multicolumn{4}{c}{~}\\
%\multicolumn{4}{c}{\textit{Total bugs found = 167}}\\
%\hline
\end{tabular}
\caption{{\small Bugs found during development using compositional testing}}
\label{tab:bugsFound}
\end{table}


==> tex/inception-bn-orca-graphs.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.32\textwidth} {
        \includegraphics[keepaspectratio=1,width=1\columnwidth]{graphs/ibn_inet_accuracy_vs_time_orca.pdf}
        \vspace{-0.25in}
        \caption{
            \label{fig:incpetion-orca-graphs-top1}
            \small
            Top-1 Accuracy vs. Time
        }
    }
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth} {
    \includegraphics[keepaspectratio=1,width=1\columnwidth]{graphs/ibn_inet_accuracy_vs_epochs_orca.pdf}
        \vspace{-0.25in}
        \caption{
            \label{fig:incpetion-orca-graphs-quality}
            \small
            Validation Accuracy vs. Epochs
        }
    }
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth} {
    \includegraphics[keepaspectratio=1,width=1.05\columnwidth]{graphs/ibn_inet_throughput_orca.pdf}
        \vspace{-0.25in}
        \caption{
            \label{fig:incpetion-orca-graphs-hardware}
            \small
            Throughput
        }
    }
    \end{subfigure}
    \vspace{-0.1in}
    \caption{
            \small
            \label{fig:incpetion-orca-graphs}
            Inception-BN on \clusterA{} trained using \imagenet{} data. 
    }
    %\vspace{-0.2in}
\end{figure*}


==> tex/layer-times-graph.tex <==
\begin{figure}[t!]
  \centering
  \begin{subfigure}{0.49\columnwidth} {
    \centerline{\includegraphics[width=1.0\columnwidth]{graphs/Inception-BN_Layer_Times_cdf.pdf}}
    \caption{
    \small
    Inception}
    \label{fig:inception-bn-imagenet-times-cdf}
  }
  \end{subfigure}
  \begin{subfigure}{0.49\columnwidth} {
    \centerline{\includegraphics[width=1.0\columnwidth]{graphs/VGG_Layer_Times_cdf.pdf}}
    \caption{
    \small
    VGG16}
    \label{fig:vgg-imagenet-times-cdf}
  }
  \end{subfigure}
  %\vspace{-0.1in}
  \caption{\small
  CDF of Layer Times
  \label{fig:layer-times-cdf}
  \deepak{Fix these graphs}
  }
  \vspace{-0.2in}
\end{figure}


==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\nocite{dean2012deepbelief, chilimbi2014adam, ngiam2011optimization, krizhevsky2014one}
\nocite{coleman2017dawnbench,ramachandran2017swish,goyal2017accurate,keskar2016large,coleman2017dawnbench,goodfellow_dlbook_:2016, bengio_practical_:2012, li_efficient_:2014}
\nocite{hadjis2016omnivore}

Others have observed that communication can often be a bottleneck for DNN training,
and worked to address it.
For example, Seide et al.\ looked at quantizing gradients~\cite{seide20141}
to decrease the amount of data needed to be communicated over the network.
Goyal et al.~\cite{goyal2017accurate} used more efficient implementations of
\texttt{all\_reduce}, like the \emph{recursive halving-and-doubling
algorithm} and the \emph{bucket algorithm} ~\cite{thakur2005optimization} to
reduce the amount of data being sent over the network. 
Others have explored techniques from the HPC literature to reduce the overhead
of communication ~\cite{baidu_performance:_2017,uber_performance:_2017}. But
all these reduction approaches still involve synchronous communication
patterns, resulting in network stalls that only slightly alleviate the
bottleneck introduced due to ever growing model sizes.

Another approach to mitigate the communication bottleneck is to allow each
machine to proceed with the next mini-batch of work before receiving the
gradients from the previous step. The gradients can be received in the
background, and are applied to the model asynchronously. 
This approach, which we call  \emph{asynchronous parallel training} (\asp{}),
improves hardware efficiency over BSP by overlapping computation with communication,
but also introduces staleness and reduces the statistical efficiency of DNN
training. Our experimental results corroborate recent findings that show that
these techniques do not reduce end-to-end DNN training time~\cite{cui2016geeps,tensorflow}.


==> tex/speedup_table.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Model / Cluster} & \textbf{\begin{tabular}[c]{@{}c@{}}Accuracy\\ threshold\end{tabular}} & \textbf{Configuration} & \textbf{\begin{tabular}[c]{@{}c@{}}Time to accuracy\\ (hours)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}End-to-end\\ speedup\\ (1 machine)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}End-to-end\\ speedup\\ (n-machine DP)\end{tabular}} \\ \toprule
\multirow{3}{*}{VGG16 / Orca} & \multirow{3}{*}{68\% top-1} & 4PP & 67.99 & 3.14 &  \\ \cmidrule(l){3-6} 
 &  & 8PP & 90.99 &  &  \\ \cmidrule(l){3-6} 
 &  & 16PP &  &  &  \\ \midrule
VGG16 / V100 & 68\% top-1 & 8PP & 13.54 & 6.98 & 5.12 \\ \midrule
Inception v3 / Orca & 67\% top-1 & 8PP & 42.88 & 7.51 & 0.99 \\ \midrule
Inception v3 / V100 & 67\% top-1 & 8PP & 25.69 & 6.87 &  \\ \midrule
s2vt / V100 & 0.294 meteor & 4PP &  &  & \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}
\caption{End-to-end speedups for different model architectures and cluster configurations. Speedups are presented for two baselines:
a single machine and the $n$-machine DP run.}
\label{my-label}
\end{table*}
